Measurements of $\Xi^{-}$ and $\overline{\Xi}^{+}$ production in proton-proton interactions at $\sqrt{s_{NN}}$ = 17.3 GeV in the NA61/SHINE experiment

The production of $\Xi(1321)^{-}$ and $\overline{\Xi}(1321)^{+}$ hyperons in inelastic p+p interactions is studied in a fixed target experiment at a beam momentum of 158 GeV/textit{c}. Double differential distributions in rapidity y and transverse momentum $p_{T}$ are obtained from a sample of 33M inelastic events. They allow to extrapolate the spectra to full phase space and to determine the mean multiplicity of both $\Xi^{-}$ and $\overline{\Xi}^{+}$. The rapidity and transverse momentum spectra are compared to transport model predictions. The $\Xi^{-}$ mean multiplicity in inelastic p+p interactions at 158~\GeVc is used to quantify the strangeness enhancement in A+A collisions at the same centre-of-mass energy per nucleon pair.

==> Makefile <==
# Makefile for generating presentation tex related files
# $Id: Makefile 3154 2013-09-26 15:17:51Z darko $

USEPDFLATEX := 1
USEBIBTEX := 1

TARGET := na61Preprint
DEPENDENCIES := $(wildcard plots/* *.tex *.bib include/*bib)

##########################################################

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

COLORIZE := awk 'BEGIN{red="\033[31;1m";yel="\033[34m";byel="\033[34;1m";end="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print red""$$0""end;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print yel""$$0""end;next}{print}END{if(w||e)print "\n"red"Warning/error summary:\n"byel""w""end;if(e)print red""e""end;exit !!e}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && exit 0 ; done ; exit 1
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $<
  bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: $(TARGET).pdf

# dependencies
$(TARGET).pdf: $(DEPENDENCIES)

clean:
	- for e in .tex~ .ps .pdf .dvi .log .toc .nav .out .snm .bbl .blg .spl .lof Notes.bib .maf .fff .lot .ttt ; do rm -f $(TARGET)$$e ; done
	- rm -f *.aux include/*.aux

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf %.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.ps
	ps2pdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<

